Twin-width and types

We study problems connected to first-order logic in graphs of bounded twin-width. Inspired by the approach of Bonnet et al. [FOCS 2020], we introduce a robust methodology of local types and describe their behavior in contraction sequences -- the decomposition notion underlying twin-width. We showcase the applicability of the methodology by proving the following two algorithmic results. In both statements, we fix a first-order formula $\varphi(x_1,\ldots,x_k)$ and a constant $d$, and we assume that on input we are given a graph $G$ together with a contraction sequence of width at most $d$. (A) One can in time $O(n)$ construct a data structure that can answer the following queries in time $O(\log \log n)$: given $w_1,\ldots,w_k$, decide whether $\phi(w_1,\ldots,w_k)$ holds in $G$. (B) After $O(n)$-time preprocessing, one can enumerate all tuples $w_1,\ldots,w_k$ that satisfy $\phi(x_1,\ldots,x_k)$ in $G$ with $O(1)$ delay. In the case of (A), the query time can be reduced to $O(1/\varepsilon)$ at the expense of increasing the construction time to $O(n^{1+\varepsilon})$, for any fixed $\varepsilon>0$. Finally, we also apply our tools to prove the following statement, which shows optimal bounds on the VC density of set systems that are first-order definable in graphs of bounded twin-width. (C) Let $G$ be a graph of twin-width $d$, $A$ be a subset of vertices of $G$, and $\varphi(x_1,\ldots,x_k,y_1,\ldots,y_l)$ be a first-order formula. Then the number of different subsets of $A^k$ definable by $\phi$ using $l$-tuples of vertices from $G$ as parameters, is bounded by $O(|A|^l)$.

==> macros_icalp.tex <==

\declaretheorem[name=Theorem,numberwithin=section]{thm}


\newcommand{\Oof}{\mathcal{O}}
\renewcommand{\preceq}{\preccurlyeq}


\newcommand{\ind}[2][]{%
  \mathrel{
    \mathop{
      \vcenter{
        \hbox{\oalign{\noalign{\kern-.3ex}\hfil$\vert$\hfil\cr
              \noalign{\kern-.7ex}
              $\smile$\cr\noalign{\kern-.3ex}}}
      }
    }^{#2}\displaylimits_{#1}
  }
}



\newcommand{\St}[1][]{\mathrm{S}^{#1}}

\linespread{1.05}
\newcommand{\from}{\colon}
\newcommand{\str}[1]{\mathbf{#1}}
\renewcommand{\cal}[1]{\mathcal {#1}}
\newcommand{\CC}{\mathscr C}
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\phi}{\varphi}






% \ifisfinalversion
	\newcommand{\limval}{\omega}
% \else
% 	\newcommand{\limval}{{\underline\omega}}
% \fi

\newcommand{\errval}{\bot}


\newcommand{\dv}[1]{\underline{#1}}
\newcommand{\D}{\mathbb D}
\newcommand{\Sym}[1]{\textrm{Sym}(#1)}


\newcommand{\approxim}[2]{\alpha_{({#1}={#2})}}
% \newcommand{\alphalow}[1]{\approxim{#1}{#1+1}}
% \newcommand{\alphalowone}[1]{\approxim{1}{2}}
% \newcommand{\alphalowtwo}[1]{\approxim{2}{3}}
% \newcommand{\alphalowthree}[1]{\approxim{3}{4}}

\newcommand{\alphalowone}{\approxim{1}{2}}
\newcommand{\alphalowthree}{\approxim{3}{4}}
\newcommand{\alphalow}[1]{
    \approxim{{#1}}{{#1}+1}
}


\newcommand{\alphahighone}{\approxim{1}{\limval}}
\newcommand{\alphahightwo}{\approxim{2}{\limval}}
\newcommand{\alphahighthree}{\approxim{3}{\limval}}
\newcommand{\alphahighfour}{\approxim{4}{\limval}}
\newcommand{\alphahighfive}{\approxim{5}{\limval}}
\newcommand{\alphahigh}[1]{
    \approxim{{#1}}{\limval}
}
\newcommand{\semidiv}[3]{{#1}{\!_{/#2=#3}}}
\newcommand{\semilow}[2]{\semidiv{#1}{#2}{#2+1}}
\newcommand{\semilowone}[1]{\semidiv{#1}{1}{2}}
\newcommand{\semilowthree}[1]{\semidiv{#1}{3}{4}}
\newcommand{\semihigh}[2]{\semidiv{#1}{#2}{\limval}}



\newcommand{\bmonoid}{\mathbb B}
\newcommand{\Bmonoid}{\overline\bmonoid}
\newcommand{\Bgamma}{\smash{\overline\bmonoid\raisebox{4.5pt}{\scriptsize$\Gamma$}}}
\newcommand{\BgammaN}{\smash{\semilow{\Bgamma\!\!\!}{N}}}
\newcommand{\BgammaNlow}[1]{{\semilow{\Bgamma\!\!\!}{#1}}}
\newcommand{\Bgammalowone}{{\semilowone{\Bgamma\!\!\!}}}
\newcommand{\BgammaNhigh}[1]{{\semihigh{\Bgamma\!\!\!}{#1}}}


\newcommand{\smonoid}{\mathbb S}
\newcommand{\Smonoid}{\overline\smonoid}
\newcommand{\Sgamma}{\smash{\overline\smonoid^\Gamma}}
\newcommand{\Sgammaone}{\smash{\overline\smonoid_1^\Gamma}}


\newcommand{\mathsym}[1]{{}}
\newcommand{\unicode}{{}}
%\newcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\smallpar}[1]{\paragraph{#1}\hspace{-3.7mm}}
%\newcommand{\smallpar}[1]{\noindent\textbf{#1}}


\newcommand{\inc}{\ensuremath{\mathit{inc}}\xspace}
\newcommand{\res}{\ensuremath{\mathit{reset}    }\xspace}
\newcommand{\chk}{\ensuremath{\mathit{check}    }\xspace}

\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\fin}{fin}
\newcommand{\qqquad}{\quad\quad\quad}
%\newcommand{\lang}{\Ll}

\newenvironment{fig}[3][!htb]%[location], file, scale, caption, label
{\begin{figure}[#1]
\centering 
\includegraphics[scale=#3]{#2}
}
{\end{figure}}
 




\newenvironment{dotlist}[0]
{\begin{list}{$\centerdot$}{}}
{\end{list}}

\newenvironment{romanlist}[0]
{\begin{list}{\makebox[0.5cm][l]{\textit{\roman{enumi})}}}{\usecounter{enumi}}}
{\end{list}}

%\newlist{enumeratep}{enumerate}{10}
%\setlist[enumeratep]{label=\quad\textit{\arabic*'.},ref=\arabic*',leftmargin=*}

% \newenvironment{enumeratep}[0]
% {\begin{list}{\makebox[0.4cm][l]{\textit{\arabic{enumi}'.}}}{\usecounter{enumi}}}
% {\end{list}}


\newenvironment{capitallist}[0]
{\begin{list}{\makebox[0.5cm][l]{{(\Alph{enumi})}}}{\usecounter{enumi}}}
{\end{list}}

\renewcommand{\labelitemi}{--}
% \newenvironment{itemize}[0]
% {\begin{list}{\makebox[0.20 cm][l]{--}}{}
% \setlength{\itemsep}{1pt}
% \setlength{\parskip}{0pt}
%  \setlength{\parsep}{0pt}
% }
% {\end{list}}

% \renewenvironment{itemize}
% {\begin{itemize}}
% {\end{itemize}}

\newenvironment{romanlist'}[0]
{\begin{list}{\makebox[0.5cm][l]{\textit{\roman{enumi}')}}}{\usecounter{enumi}}}
{\end{list}}

%idziaszek

\newcommand{\savelabel}[2]{\expandafter\newtoks\csname#1\endcsname
  \global\csname#1\endcsname={#2} \label{#1} #2}
\newcommand{\loadlabel}[1]{\noindent {\bf Lemma~\ref{#1}. } \textit{\the\csname#1\endcsname}
\medskip

}
\renewcommand{\setminus}{-}%{\rotatebox[origin=c]{-20}{--- }}

\newcommand{\loadlabelthm}[1]{\medskip\noindent {\bf Theorem~\ref{#1}. }
  \noindent  \textit{\the\csname#1\endcsname}
\medskip
}

\newcommand{\idziaszek}[1]{\loadlabelthm{#1}}


\newcommand{\loadlabelprop}[1]{\noindent {\bf Proposition~\ref{#1}. }
  \noindent  \textit{\the\csname#1\endcsname}
\medskip

}


\newenvironment{tablist}[0]
{\medskip\vspace{5pt}
\begin{tabular}{ll}}
{\end{tabular}\medskip\vspace{5pt}\newline}


\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Nbar}{\overline{\N}}
\newcommand{\Qbar}{\overline{\Q}}
\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\eps}{\varepsilon}
\newcommand{\preim}[2]{#1^{-1}(#2)}
\newcommand{\sgn}[0]{\mathrm{Sgn}}
% \newcommand{\underbracel}[1]{\mathop{\mathchoice{%
%     \underbrace{disp\displaystyle#1}}{%
%     \underbrace{text\textstyle#1}}{%
%     \underbrace{\scriptstyle#1}}{%
%     \underbrace{\scriptscriptstyle#1}
%   }}\limits}

\newcommand{\func}[3]{\mathop{\mathchoice{%
    {#1}\quad\colon\quad{#2}\quad\longrightarrow\quad {#3}}{%
    {#1}\colon{#2}\to{#3}}{%
    script}{%
    sscript}
  }}



% newcommand{\func}[3]{\mathop{\mathchoice{
% 	{{#1}\quad\colon\quad {#2}\quad\longrightarrow\quad {#3}}{${#1}\colon{#2}\to{#3}$}{${#1}\colon{#2}\to{#3}$}{${#1}\colon{#2}\to{#3}$}}}}
%\newcommand{\func}[3]{\mbox{${#1}\colon{#2}\to{#3}$}} %function
\newcommand{\wlozenie}[3]{\mbox{$#1\colon#2\hookrightarrow#3$}} %embedding
\newcommand{\razy}{\cdot}
\newcommand{\zloz}{\circ}
\newcommand{\cp}[0]{\smallsmile}
\newcommand{\id}{\iota}
\newcommand{\tryw}{\mathbbm{1}} %grupa trywialna -- poprawic
\newcommand{\lie}[1]{\mathfrak{#1}}
\renewcommand{\subset}{\subseteq}
\newcommand{\tensor}{\otimes}
\newcommand{\qlor}{\ \lor\ }
\newcommand{\qland}{\ \land\ }

\newcommand{\fotwo}{{$\mathsf{FO_2}$}}
\newcommand{\fo}{{{\textsf{FO}}}}
\newcommand{\V}{\mathcal V} %green's relations
\newcommand{\J}{\mathcal J}
\renewcommand{\H}{\mathcal H}
\newcommand{\inv}[2]{#1^{-1}(#2)}
\newcommand{\rel}{\sim}
\newcommand{\prof}[1]{{\widehat{{#1}^+}}}
\newcommand{\var}{\ensuremath{\mathbf V}\xspace}
\newcommand{\profv}[1]{{\widehat{{#1}^+_{\var}}}}
%\newcommand{\profv}[1]{dupa}%{{\overline{\Omega_\var{#1}}}}
\newcommand{\profs}[1]{{\widehat{{#1}^*}}}
\newcommand{\Pc}{P_c}
\newcommand{\lang}[1]{L\left({#1}\right)}

\newcommand{\logspace}{\textsc{LogSpace}\xspace}%{$\mathbf{PSPACE}$}
\newcommand{\pspace}{\textsc{PSpace}\xspace}%{$\mathbf{PSPACE}$}
\newcommand{\ptime}{\textsc{PTime}\xspace}%{$\mathbf{PSPACE}$}
\newcommand{\expspace}{\textsc{ExpSpace}\xspace}%{$\mathbf{PSPACE}$}
\newcommand{\npspace}{\textsc{NPspace}}%{$\mathbf{PSPACE}$}
\newcommand{\exptime}{\textsc{Exptime}}%{$\mathbf{PSPACE}$}



\renewcommand{\S}{{\infty}}
%\newcommand{\B}{{<\infty}}
\newcommand{\B}{{\mathchoice
	{%displaystyle
	<\!\!\infty
    }{%textstyle
	<\!\!\infty
    }{%scriptstyle
	<\infty
    }{%scriptscriptstyle
	<\infty
    }
}
}




\newcommand{\atleast}[1]{{\ge n}}
\newcommand{\less}[1]{{<n}}


%\newcommand{\nota}[1]{\-\marginpar[\raggedleft\footnotesize #1]%
%{\raggedright\footnotesize #1}}




%\ifisfinalversion
	\newcommand{\notacol}[2]{}
% \else
 	%\newcommand{\notacol}[2]{\mbox{}\marginpar{\footnotesize\raggedright\hspace{0pt}\color{#2}\textit{#1}}}
% \fi

 \newcommand{\nota}[1]{\notacol{@@#1}{blue}}
 \newcommand{\unfinished}{\notacol{@@unfinished}{red}}
 \newcommand{\checknotation}[1]{\notacol{@@#1}{green}}



\newcommand{\definp}[2]{\emph{#1}\index{#2}}%\notacol{#2}{black}}
\newcommand{\defin}[1]{\definp{#1}{#1}}
\newcommand{\definr}[1]{#1\index{#1}}%\notacol{#1}{black}}


%\newcommand{\nota}[1]{\mbox{}\marginpar{\footnotesize\raggedright\hspace{0pt}\color{blue}\textit{#1}}}

%\newcounter{quote}
\newsavebox{\quoteitbox}

\newenvironment{quoteit}[1] 
{\begin{sloppypar}\noindent\slshape\sbox{\quoteitbox}{#1}\begin{quote}\itshape}%
{\hspace*{\fill}{\upshape(\usebox{\quoteitbox})}\end{quote}%
\end{sloppypar}\noindent\ignorespacesafterend}

\newenvironment{quoteit*} 
{\begin{sloppypar}\noindent\slshape\begin{quote}\itshape} 
	{\end{quote}\ignorespaces\end{sloppypar}\noindent\ignorespacesafterend}



\newenvironment{quotetag}[1][]
{~\par%\vskip 0mm                % Skip down 1/2 before story
	\begingroup                  % Start of formatting properties
	%\rightskip4em\leftskip4em   % Wider margins for narrower text
	\begin{equation}
		 \ifthenelse{\equal{#1}{}}{}{\tag{#1}}
		 \begin{minipage}[c]{115mm}
			\it                          % Italic font
	%		\noindent{\par}  % Make dotted line
			\noindent{\par}
			\begin{center}
}
{
        \end{center}
		\end{minipage}
	\end{equation}
	%\par%\noindent{\par}  % Make dotted line
	\endgroup                        % End of formatting properties
%~\vskip 0mm                    % Skip final 1/2 inch}
\par
\medskip
}

\newenvironment{quotetag*}
{~\par%\vskip 0mm                % Skip down 1/2 before story
	\begingroup                  % Start of formatting properties
	\begin{equation*}
		 \begin{minipage}[c]{115mm}
			\it\noindent{\par}
}
{
		\end{minipage}
	\end{equation*}
	\endgroup                        % End of formatting properties
\par
\textnormal
\medskip
}

%% Caligraphic

\newcommand{\Aa}{\ensuremath{\mathcal A}\xspace}
\newcommand{\Bb}{{\mathcal B}}
\newcommand{\Cc}{{\mathcal C}}
\newcommand{\Dd}{\ensuremath{\mathcal D}\xspace}
\newcommand{\Ee}{{\mathcal E}}
\newcommand{\Ff}{{\mathcal F}}
\newcommand{\Gg}{{\mathcal G}}
\newcommand{\Hh}{{\mathcal H}}
\newcommand{\Jj}{{\mathcal J}}
\newcommand{\Kk}{{\mathcal K}}
\newcommand{\Ll}{{\mathcal L}}
\newcommand{\Mm}{{\mathcal M}}
\newcommand{\Nn}{{\mathcal N}}
\newcommand{\Oo}{{\mathcal O}}
\newcommand{\Pp}{{\mathcal P}}
\newcommand{\Qq}{{\mathcal Q}}
\newcommand{\Rr}{{\mathcal R}}
\newcommand{\Ss}{{\mathcal S}}
\newcommand{\Tt}{{\mathcal T}}
\newcommand{\Uu}{{\mathcal U}}
\newcommand{\Vv}{\ensuremath{\mathcal V}\xspace}
\newcommand{\Ww}{{\mathcal W}}
\newcommand{\Xx}{{\mathcal X}}
\newcommand{\Yy}{{\mathcal Y}}
\newcommand{\Zz}{{\mathcal Z}}


\newcommand\set[1]{\ensuremath{\{#1\}}}
\newcommand{\setof}[2]{\set{#1\mid#2}}


\DeclareMathOperator{\tp}{tp}
\newcommand{\tup}[1]{{\mathbf{#1}}}


%%%defined by some layouts

\newtheoremstyle{theoremstyle}% name of the style to be used
  {3pt}% measure of space to leave above the theorem. E.g.: 3pt
  {3pt}% measure of space to leave below the theorem. E.g.: 3pt
  {\itshape}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\bfseries}% name of head font
  {.}% punctuation between head and body
  {4pt}% space after theorem head; " " = normal interword space
  {}% Manually specify head


%\theoremstyle{theoremstyle}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem*{theorem*}{Theorem}
%\newtheorem*{tropicaltheorem}{Theorem $(\star)$}
%\newtheorem{tw}{Twierdzenie}
%\newtheorem{lemma}[theorem]{Lemma}%[chapter]
%\newtheorem{corollary}[theorem]{Corollary}%[chapter]
%\newtheorem{proposition}[theorem]{Proposition}%[chapter]
%\newtheorem{claim}{Claim}
%\newtheorem{hypo}{Hypothesis}
%\newtheorem{fact}{Fact}
%\newtheorem{observation}{Observation}

\newtheoremstyle{remarkstyle}% name of the style to be used
  {3pt}% measure of space to leave above the theorem. E.g.: 3pt
  {10pt}% measure of space to leave below the theorem. E.g.: 3pt
  {}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\itshape}% name of head font
  {}% punctuation between head and body
  {4pt}% space after theorem head; " " = normal interword space
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}.}% Manually specify head


\theoremstyle{remarkstyle}
%\newtheorem{example}{Example}[section]
\newtheorem{przykl}{Przykład}
%\newtheorem{remark}{Remark}[section]
\newtheorem{notation}{Notation}[section]

\newtheoremstyle{definitionstyle}% name of the style to be used
  {3pt}% measure of space to leave above the theorem. E.g.: 3pt
  {3pt}% measure of space to leave below the theorem. E.g.: 3pt
  {}% name of font to use in the body of the theorem
  {0pt}% measure of space to indent
  {\bfseries}% name of head font
  {}% punctuation between head and body
  {4pt}% space after theorem head; " " = normal interword space
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}.}% Manually specify head


\theoremstyle{definitionstyle}
%\newtheorem{definition}{Definition}


\numberwithin{equation}{section}
\renewcommand{\theequation}{\arabic{equation}}




\newcommand*\mycirc[1]{%
  \begin{tikzpicture}[baseline=(C.base)]
    \node[draw,circle,inner sep=0.5pt](C) {#1};
  \end{tikzpicture}}






\newcommand{\name}[1]{{#1}\xspace}


%%%specific to paper

\newcommand{\matr}[2]{\mathbb M_{#1}#2}
\newcommand{\mat}{\mathbb{M}}

\newcommand{\M}{\mathbb{M}}


\newcommand{\unbound}{\ensuremath{\mathsf U}\xspace}
\newcommand{\bound}{\ensuremath{\mathbb B}\xspace}
\newcommand{\rec}{\ensuremath{\mathsf R}\xspace}
%\newcommand{\bound}{\ensuremath{\mathsf B}\xspace}
\newcommand{\per}{\ensuremath{\mathsf P}\xspace}
\newcommand{\efin}{{\exists_{\mathsf{fin}}}}

\newcommand{\invlim}{\underleftarrow \lim}
%\newcommand{\stab}[1]{#1^\#}
\newcommand{\stab}[0]{\#}
\newcommand{\stabsize}[1]{|\!|#1|\!|}
%\newcommand{\stabcl}[1]{#1^{+,\#}}
%\newcommand{\omcl}[1]{#1^{+,\omega}}
% \newcommand{\stabcl}[1]{\mathit{Gen}(#1,\ \cdot \ ,\stab)}
% \newcommand{\omcl}[1]{\mathit{Gen}(#1,\ \cdot \ ,\omega)}
\newcommand{\stabcl}[1]{#1^{\langle\; \cdot\; ,\#\rangle}}
\newcommand{\omcl}[1]{#1^{\langle\;\cdot\; ,\omega\rangle}}
% \newcommand{\stabcl}[1]{\mathit{Gen}_{\langle\;\cdot\;,\stab\rangle}A}
% \newcommand{\omcl}[1]{\mathit{Gen}_{\langle\;\cdot\;,\omega\rangle}A}

\newlength{\wideaslength}

\newcommand{\wideas}[2]{\settowidth{\wideaslength}{{#1}}%
\makebox[\wideaslength][c]{#2}%
}


% \newlength{\pluswidth}
% \settowidth{\pluswidth}{${}+{}$}

%\makebox[\tmpwidth][s]{$m\cdot n$}
\newcommand{\opdot}{\wideas{${}+{}$}{$\cdot$}}%{\makebox[\pluswidth][c]{$\cdot$}}
\newcommand{\sigdot}{\; \cdot\;}

\newcommand{\syntmap}{{\sigma}}
\newcommand{\omsignature}{{\ensuremath{\langle\sigdot ,\omega\rangle}}}
\newcommand{\stabsignature}{{\ensuremath{\langle\sigdot ,\stab\rangle}}}
\newcommand{\dotsignature}{{\langle\sigdot \rangle}}
\newcommand{\skappa}{\langle\sigdot,\stab\rangle}


\newcommand{\app}{$\spadesuit$}
\newcommand{\der}[2]{#1^{(#2)}}
\newcommand{\rH}{\sim_{\mathcal H}}
\newcommand{\rL}{\sim_{\mathcal L}}
\newcommand{\rR}{\sim_{\mathcal R}}
\newcommand{\rD}{\sim_{\mathcal R}}
\newcommand{\ultper}{\mathsf{P}}
\renewcommand{\subset}{\subseteq}
\newcommand{\cld}{\downarrow\!}
\newcommand{\clu}{\uparrow\!}

\newcommand{\dist}{{\mathrm{dist}}}
\newcommand{\Oh}{\mathcal{O}}

\newcommand{\w}{\ensuremath{\omega}}
\newcommand{\Tropical}{\Tt}
\newcommand{\wB}{$\omega$B}
\newcommand{\wS}{$\omega$S}
\newcommand{\wBS}{$\omega$BS}
\newcommand{\ass}[2]{{#1:=#2}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Pd}{P_\downarrow}
\newcommand{\Pu}{P_\uparrow}
\newcommand{\conv}{conv}

\newcommand{\condB}[1]{B(#1)}
\newcommand{\condS}[1]{S(#1)}

\newcommand{\data}{\mathbf D}

\newcommand{\mso}{{\upshape MSO}\xspace}
\newcommand{\msou}{{\upshape MSO}+\unbound}
\newcommand{\msob}{{\upshape MSO}+\bound}
\newcommand{\wmsou}{Weak{\upshape MSO}+\unbound}
\newcommand{\wmsour}{Weak{\upshape MSO} \!+\textsf{U}+\textsf{R}\xspace}
%\newcommand{\msop}{\mso\!$_+$}
\newcommand{\msoinf}{{\upshape MSO}+$\inf$\xspace}
\newcommand{\msopinf}{\textrm{\upshape MSO}+$\inf^\text{+}$\xspace}
\newcommand{\msopfin}{\textrm{\upshape MSO}+$\fin^\text{+}$\xspace}
\newcommand{\op}[1]{\textrm{Op}_{#1}}

\newcommand{\seta}[1]{}
\newcommand{\as}[1]{\underline {#1}}
\newcommand{\As}[1]{\underline {#1}}
\newcommand{\partiso}[1]{\textit{Partial}(#1)}
\newcommand{\partisofin}[1]{\textit{FinPartial}(#1)}
\newcommand{\iso}[2]{\textit{Iso}_{#1}(#2)}
\newcommand{\dom}[1]{\textrm{Dom}(#1)}
\renewcommand{\im}[1]{\textrm{Im}(#1)}


\newcommand{\val}[2]{\mathit{val}_{#1}\!\left(#2\right)}
\newcommand{\maxval}[2]{\mathit{maxval}_{#1}\!\left(#2\right)}

\newcommand{\add}[2]{\mathbf{\Sigma}_{#2}}
\newcommand{\mult}[2]{\mathbf{\Pi}_{#2}}
\newcommand{\amb}[2]{\mathbf{\Delta}_{#2}}
\newcommand{\bool}[1]{\mathcal{BC}_{#1}}

\newcommand{\fromto}[2]{\textit{#1\;$\Rightarrow\;\!$#2}.\quad\ignorespaces}
\newcommand{\fromtoboth}[2]{\textit{#1\;$\Leftrightarrow\;\!$#2}.\quad\ignorespaces}
\newcommand{\fromtodouble}[3]{\textit{#1\;$\Rightarrow\;\!$#2 \& #3}.\quad\ignorespaces}
\newcommand{\fromtosub}{{($\subseteq$)}.\ }
\newcommand{\fromtosup}{{($\supseteq$)}.\ } 
\newcommand{\fromtoleq}{{($\leq$)}.\ }
\newcommand{\fromtogeq}{{($\geq$)}.\ }


\newcommand{\eqdef}{\quad\stackrel{\mathit{def}}{=}\quad}
\newcommand{\jclass}{{$\mathcal J$-class }}
\def\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$<$}}}                % less than or approx. symbol

\newcommand{\contr}{\!\uparrow^}
\newcommand{\sat}{\vDash}
\definecolor{gray1}{rgb}{0.99,0.99,0.99}
\definecolor{gray2}{rgb}{0.97,0.97,0.97}
\definecolor{gray3}{rgb}{0.95,0.95,0.95}
\definecolor{gray4}{rgb}{0.93,0.93,0.93}
\definecolor{gray5}{rgb}{0.91,0.91,0.91}
\definecolor{gray6}{rgb}{0.89,0.89,0.89}
\definecolor{gray7}{rgb}{0.87,0.87,0.87}
\definecolor{gray8}{rgb}{0.85,0.85,0.85}
\definecolor{gray9}{rgb}{0.83,0.83,0.83}
\definecolor{gray10}{rgb}{0.81,0.81,0.81}
\definecolor{gray20}{rgb}{0.71,0.71,0.71}
\definecolor{gray40}{rgb}{0.51,0.51,0.51}


\newcommand{\ERCagreement}{%partially supported by the $111$ project of the Ministry of Education of China.
\vspace{-6pt}

\noindent
{\begin{minipage}[t]{\textwidth}\small This paper is a part of project {\sc{BOBR}} that has received funding from the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation programme (grant agreement No 948057). \end{minipage}\hfill

\begin{minipage}{.32\textwidth}\includegraphics[width=\textwidth]{ERC2}\end{minipage}\hfill}}

\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}


\def\cqedsymbol{\ifmmode$\lrcorner$\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil$\lrcorner$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi} 
\newcommand{\cqed}{\renewcommand{\qed}{\cqedsymbol}}


==> omitted-proofs.tex <==
\section{Omitted proofs}\label{sec:omitted}

In this appendix we provide proofs omitted in the main body of the paper.

\subsection{Omitted proofs from Section~\ref{sec:prelims}}

\subsection{Omitted proofs from Section~\ref{sec:types}}

\subsection{Omitted proofs from Section~\ref{sec:queries}}



==> packages_icalp.tex <==
%\usepackage[english]{babel}
\usepackage{hyperref}

\usepackage{amsmath, amsfonts,xfrac, amsthm,amssymb}

\usepackage{mathtools}

%\usepackage{setspace}

%\usepackage{geometry}
%\usepackage{xypic,colortbl}


\usepackage{thmtools}
%\usepackage{thm-restate}

% \usepackage[usenames]{color}

%\usepackage{microtype}

%\usepackage{enumitem}

%\usepackage{sidecap}

%\usepackage{wrapfig}


\usepackage{ifthen, xspace}

\usepackage{mathrsfs, stmaryrd}

%\usepackage{sectsty}

\usepackage{
 calc, makeidx,bbold
}%showidx, bbold

\usepackage[font=small,format=plain,labelfont=sc,textfont=it]{caption}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[all]{xy}
%\usepackage[geometry]{ifsym}
\usepackage[cmyk]{xcolor}

\usepackage{palatino}
%\usepackage{mathpazo}
\usepackage{comment}

\usepackage{todonotes}

\usepackage{textpos}


